Monolithic MHz-frame rate digital SiPM-IC with sub-100 ps precision and 70$~\mu$m pixel pitch

This paper presents the design and characterization of a monolithic integrated circuit (IC) including digital silicon photomultipliers (dSiPMs) arranged in a 32$~\times~$32 pixel matrix at 70$~\mu$m pitch. The IC provides per-quadrant time stamping and hit-map readout, and is fabricated in a standard 150-nm CMOS technology. Each dSiPM pixel consists of four single-photon avalanche diodes (SPADs) sharing a quenching and subsequent processing circuitry and has a fill factor of 30$~\%$. A sub-100$~$ps precision, 12-bit time-to-digital converter (TDC) provides timestamps per quadrant with an acquisition rate of 3$~$MHz. Together with the hit map, the total sustained data throughput of the IC amounts to 4$~$Gbps. Measurements obtained in a dark, temperature-stable environment as well as by using a pulsed laser environment show the full dSiPM-IC functionality. The dark-count rate (DCR) as function of the overvoltage and temperature, the TDC resolution, differential and integral nonlinearity (DNL/INL) as well as the propagation-delay variations across the matrix are presented. With aid of additional peripheral test structures, the main building blocks are characterized and key parameters are presented.

==> design.tex <==
	\section{Chip architecture} \label{sec:design}
	\subsection{Matrix and periphery}
	The monolithic IC (cf. figure~\ref{fig:chip}a) has been designed in LFoundry's 150-nm CMOS technology to take advantage of an available add-on library including single p+/nwell SPADs with an active area of 20~$\times$~20~$\mu$m$^{2}$. This area is framed by a cathode ring plus an additional pwell ring to minimize the crosstalk to neighboring cells. The dSiPM-pixel design comprises four SPADs in parallel sharing the pwell ring and using it partially for the NMOS transistors of the common pixel electronics to reduce dead area. In this way, the pixel covers an area of 69.6~$\times$~76~$\mu$m$^{2}$ with a fill factor of 30~$\%$. Figure~\ref{fig:chip} shows the layout of the IC (a) and a photograph of the dSiPM pixel (b).
%	In HEP experiments, this fill factor has a negative impact on direct MIP detection efficiency, as it will be discussed in~\cite{dSiPMTB}, but this constraint could be solved by a scintillator on top of the sensor matrix or by using two staggered sensor layers.

\begin{figure}[h]
	\centering
	\includegraphics[width=0.93\linewidth]{N:/4all/public/fec/Projects/APD/Presentations and Meetings/dSiPM-ASICpaper_2023/arXiv/Layout+Foto_v3}
	\put(-410,264){\makebox(0,0){a)}} 	\put(-108,154){\makebox(0,0){b)}}
	\caption{a) IC layout (3400~$\times$~3300~$\mu$m$^{2}$). b) dSiPM-pixel photograph (69.6~$\times$~76~$\mu$m$^{2}$).}
	\label{fig:chip}
\end{figure}
	
	The IC consists of four identical units (quadrants), each one (cf. figure~\ref{fig:ROscheme}) with a 16~$\times$~16 dSiPM-pixel matrix, a single 12-bit TDC for event-time stamping, a validation logic with adjustable settings for discarding undesirable events, and serializer circuits followed by links (MUX~+~TX) for fast (about 1~Gbps) and sustained data readout. In this way, the system provides the full hit map of a 32~$\times$~32~dSiPM-pixel matrix together with four timestamps for each frame.
		
	\begin{figure}[htb]
		\centering
		\includegraphics[width=1\linewidth]{N:/4all/public/fec/Projects/APD/Presentations and Meetings/dSiPM-ASICpaper_2023/Pics/Readout_v2}
		\caption{Quadrant block diagram.}
		\label{fig:ROscheme}
	\end{figure}
	
	Figure~\ref{fig:ROscheme} shows a simplified block diagram of one quadrant with all components, as well as additional blocks used globally for all quadrants. 
	When an avalanche process is initiated in a SPAD, the pixel draws current from a fast wired-OR connection, and the earliest pixel in the readout frame triggers the TDC. Simultaneously, the row-wise wired-ORs are monitored by a validation logic generating a valid bit for this event. The latched outputs of a peripheral 40-bit frame counter (FC) complete the quadrant timing information with the frame number of the event. The TDC and FC are started by the \emph{Shutter} signal defining the beginning of a measurement. The 40-bit FC allows a total recording time of about 100~hours for a measurement. The timing data are serialized and multiplexed together with the timing data of the other quadrants. The counted hits in each pixel are serialized row-wise and multiplexed column-wise to deliver the hit map of the quadrant. 
	In the periphery, an initialization register provides the control signals for pixel masking, validation thresholds and TDC settings. Furthermore, clock dividers and buffers serve to distribute all essential clocks to the components. The main clocks are provided by the DAQ system. The frame-based readout and operation mode runs at a targeted frequency of 3~MHz (\emph{FRAME CLK}). Additionally, a 408-MHz \emph{SYSTEM CLK} (multiple of the \emph{FRAME CLK}) is required as reference clock for the TDCs (cf. \emph{TDC Ref Clock}) as well as for the multiplexers to enable the sustained readout of the entire hit matrix.

	\subsection{Block details and timing}
\begin{figure}
	\centering
	\includegraphics[width=.9\linewidth]{N:/4all/public/fec/Projects/APD/Presentations and Meetings/dSiPM-ASICpaper_2023/Pics/PixelValid}
	\put(-400,120){\makebox(0,0){a)}} 	\put(-155,120){\makebox(0,0){c)}}
	\qquad
	\centering
	\includegraphics[width=1\linewidth]{N:/4all/public/fec/Projects/APD/Presentations and Meetings/dSiPM-ASICpaper_2023/Pics/TDCv2}
	\put(-420,170){\makebox(0,0){b)}}
	\qquad
	\caption{Simplified equivalent circuits of: a) the dSiPM pixel, b) the TDC, and c) the validation logic.}
	\label{fig:circuits}
\end{figure}
	
	Figure~\ref{fig:circuits}a shows the dSiPM-pixel electronics consisting of the four SPADs connected in parallel, a front-end circuitry using 3.3-V NMOS transistors, and a readout circuitry operating at core voltage of 1.8~V. The front end allows an overvoltage (V$_{ov}$) of maximally 3.6~V, which sets the anode voltage. The used quenching circuit is similar to the presented one in~\cite{7066818}, where the quenching is performed by a globally biased transistor (cf. \emph{V$_{Quench}$}) and an inverter (cf. INV) as comparator for the digital pulse shaping (cf. \emph{Out}). A clamping transistor (cf. \emph{V$_{Clamp}$}) limits the inverter input to 1.8~V. The pixel electronics include the possibility to mask a pixel (cf. \emph{Masking}) via a single SRAM cell. The hold-off time of the pixel can be adapted by the global bias voltage \emph{V$_{Quench}$}. Detected hits can be counted within the acquisition window by the 2-bit hit counter. If this function is not needed, the counter can be set as buffer by the control signal \emph{/Set$\_$2bit}.
	
	Figure~\ref{fig:circuits}b shows the TDC, which is divided into a fine and coarse converter. The fine TDC consists of a delay-locked loop (DLL) with 32 differential delay elements (DEs). A phase-frequency detector compares the incoming reference signal (cf. \emph{Rf}) with the delayed one (cf. \emph{Dl}) and steers the following charge pump like in~\cite{DLL}. The resulting voltage over the loop-filter capacitance (C$_{LF}$) together with a calibration circuit controls the delay of all DEs (cf. \emph{V$_{c}$}). The DE outputs are latched by the wired-OR trigger signal until the next frame starts. The latched signals are encoded as thermometer code and have to be decoded into binary with the aid of a 32-to-5-bit encoder. After each DLL cycle, a subsequent ripple counter is incremented and serves as 7-bit coarse TDC.
	
	The row-wise wired-OR outputs (cf. \emph{R<0:15>}) are monitored by a 4-step validation logic generating a valid bit for an event, as displayed in figure~\ref{fig:circuits}c. In the first validation step, every row output is connected by a selectable AND/OR gate with its neighboring row output. In each subsequent step all gates in a column can be programmed as AND or OR (by \emph{Valid$\_$cntr<0:3>}). In this way, pixel in a cluster of few pixels firing simultaneously can be identified. 
		
	\begin{figure}[h]
		\centering
			\includegraphics[width=1\linewidth]{N:/4all/public/fec/Projects/APD/Presentations and Meetings/dSiPM-ASICpaper_2023/Pics/Signals}
		\caption{Timing diagram of the frame-based readout.}
		\label{fig:Timing}
	\end{figure}

 	Figure~\ref{fig:Timing} shows the underlying timing diagram with input clocks, internal signals and output data for the hit counter set in 1-bit mode. The acquisition window is defined by the rising edge of \emph{Frame$\_$rst} and the falling edge of \emph{Read}. Afterwards, all collected data are buffered into the serializers and read out during the following frame. The dynamic range of the TDC with $2^{7}$/408~MHz~=~313.7~ns corresponds to the acquisition window. By using the hit counter in 2-bit mode, the readout time has to be adapted to enable full hit-map readout. Accordingly, the acquisition window extends to two frame-clock cycles.
 	
 	\subsection{Test circuits}
 	
 	In the periphery of the matrix, test circuits are integrated for single-block characterization (cf. figure~\ref{fig:chip}a). These extra blocks comprise a stand-alone TDC, as well as a chain of receiver~(RX) and transmitter~(TX) links using the low-voltage differential signaling~(LVDS) standard. The simplified block schemes are shown in figure~\ref{fig:RXTX}. The RX consists of a Schmitt-Trigger circuitry operated at 3.3~V supply voltage and is followed by a voltage-conversation stage delivering single-ended output. The TX includes an input stage comprising an edge aligner, voltage converter and buffers to drive the input of the subsequent current-switching circuitry. To keep the output common mode stable about 1.2~V, a common-mode feedback (CMFB) steers the output current. Both circuits are terminated with 100~$\Omega$ on the chip.
 		
\begin{figure}[h]
	\centering
	\includegraphics[width=1\linewidth]{N:/4all/public/fec/Projects/APD/Presentations and Meetings/dSiPM-ASICpaper_2023/Pics/RX_TX}
	\caption{Simplified block diagrams of the RX and TX.}
	\label{fig:RXTX}
\end{figure}
 	Additionally, sensor-test structures in different configurations are implemented. For example, a 3~$\times$~3~test-SPAD array, where the center SPAD is connected to the same front end as used for the dSiPM pixel, enables the monitoring of the digital output of a single SPAD.

